Multi-Agent Dynamic Pricing in a Blockchain Protocol Using Gaussian Bandits

The Graph Protocol indexes historical blockchain transaction data and makes it available for querying. As the protocol is decentralized, there are many independent Indexers that index and compete with each other for serving queries to the Consumers. One dimension along which Indexers compete is pricing. In this paper, we propose a bandit-based algorithm for maximization of Indexers' revenue via Consumer budget discovery. We present the design and the considerations we had to make for a dynamic pricing algorithm being used by multiple agents simultaneously. We discuss the results achieved by our dynamic pricing bandits both in simulation and deployed into production on one of the Indexers operating on Ethereum. We have open-sourced both the simulation framework and tools we created, which other Indexers have since started to adapt into their own workflows.

==> _other.tex <==
THE VALUE OF SIMULATION - purposes: These purposes include prediction, performance, training, entertainment,
education, proof, and discovery~\cite{axelrod1997advancing}

Proof. Simulation can be used to provide an existence proof. For example, Conway’s Game of Life demonstrates that extremely complex behavior can result from very simple rules [2].

% More from \cite{axelrod1997advancing}
%Simulation can be compared with the two standard methods of induction and deduction. Induction is the discovery of patterns in empirical data. For example, in the social sciences, induction is widely used in the analysis of opinion surveys and the macroeconomic data. Deduction, on the other hand, involves specifying a set of axioms and proving consequences that can be derived from those assumptions. The discovery of equilibrium results in game theory using rational choice axioms is a good example of deduction.
%Simulation is a third research methodology. Like deduction, it starts with a set of explicit assumptions. But unlike deduction, it does not prove theorems. Instead, simulation generates data that can be analyzed inductively. Unlike typical induction, however, the simulated data come from a specified set of rules rather than direct measurement of the real world. While induction can be used to find patterns in data, and deduction can be used to find consequences of assumptions, simulation modeling can be used to aid intuition.

agent-based modeling (ABM) can address research questions common to many disciplines~\cite{axelrod2006agent}

formulate and test a series of theorems about the conditions under which cooperation based upon reciprocity can emerge in a population of egoists, and then resist invasion by mutant strategies.


Since its inception in the early 1990s [17, 31, 36], Agent-Based Simulation (ABS) as a third way of doing science [3, 5] has matured substantially and has found its way into the mainstream of science [25].~\cite{macal2016everything}

\textbf{Contributions}: The contributions of this paper are:

\begin{itemize}
    \item No contributions - no paper! TODO!
    \item emphasize The Graph as one of the most complex protocols, with complex on- and off-chain logic
\end{itemize}

lack of clear requirements (profit maximization?) -> ABS and formulation of desired outcomes in terms of isolated agent properties tested against various market conditions and or other agents helps!

Solving two problems:
\begin{itemize}
    \item with RL - trying to maximize the revenue in dynamic and competitive environment
    \item with ABM - trying to make sure that QoS is OK (queries are served) and agents are not starving/making money
\end{itemize}


\subsection{The Graph Scenario}

The considered scenario is presented in fig.~\ref{fig:scenario} - focus on query serving and payments.


Customers send queries to The Gateway.
The Gateway distributes queries between indexers.
The decision is based on each indexer’s price-bid and it’s quality of service.
Indexers earn money by serving queries.
Indexers can control the prices of served queries.

The whole system can be perceived as a \textbf{Game}: Agent’s revenue maximization vs Gateway’s quality of service.


Price bids expressed as models in DSL called Agora

AutoAgora = Dynamic pricing based on query volume received by an indexer.


\begin{itemize}
\item Queries distributed amongst agents depending on their price bids (the same)
\item All Indexers should have freedom with their pricing models
\item All Indexers should be able to make (some) profit
\end{itemize}

MARL~\cite{busoniu2008comprehensive,zhang2021multi}



==> backup.tex <==
\section{Problem Formulation Backup}

In our simulation we've made several assumptions that led to the simplified scenario presented in \autoref{fig:simulation}.
First, we have decided to abstract from the customers and types of GraphQL queries.
Instead we simulate the traffic as a total query volume that the indexers have to handle in a given time interval ($q/s$).
As a consequence, we assume that all the queries in a given volume are associated with exactly the same budget.
Finally, we do not consider the costs of serving queries, hence the agents operate purely on revenue calculated one the base of served traffic multiplied by the unit price.
\subsection{Agents}
There are several types of agents used in our experiments.
Most important ones are \textbf{Gaussian bandits}, i.e. trainable, stochastic agents with policy represented as a Gaussian distribution over the continuous query price space.
The bandits~\cite{lattimore2020bandit} have no internal representation of the environment and during operation agent's actions are sampled from the policy distribution.
In most of our experiments we use a slightly modified version proximal policy optimization~\cite{schulman2017proximal} for updating agent's policies.

In some of the experiments we compare performance of our Gaussian bandits with heuristic agents of two types: deterministic agents with fixed prices and stochastic agents with fixed Gaussian distributions.

% policy gradients~\cite{peters2006policy,kakade2001natural,sutton1999policy}
%Trainable (RL)~\cite{sutton2018reinforcement} vs Rule-based (i.e. with predefined behaviors)





